Joint discrete and continuous matrix distribution modelling

In this paper we introduce a bivariate distribution on $\mathbb{R}_{+} \times \mathbb{N}$ arising from a single underlying Markov jump process. The marginal distributions are phase-type and discrete phase-type distributed, respectively, which allow for flexible behavior for modeling purposes. We show that the distribution is dense in the class of distributions on $\mathbb{R}_{+} \times \mathbb{N}$ and derive some of its main properties, all explicit in terms of matrix calculus. Furthermore, we develop an effective EM algorithm for the statistical estimation of the distribution parameters. In the last part of the paper, we apply our methodology to an insurance dataset, where we model the number of claims and the mean claim sizes of policyholders, which is seen to perform favorably. An additional consequence of the latter analysis is that the total loss size in the entire portfolio is captured substantially better than with independent phase-type models.

==> Dataset1.tex <==
\subsection{Application: Insurance Data}
The dataset \texttt{freMTPLsev} contains claims for insurance policies. The policies have from 1-4 claims, and there are in total $15300$ policies. Table \ref{tab:sumstat} gives an overview of the data. 
\begin{table}[H]
    \centering
    \begin{tabular}{c|c c c c}
         Number of Claims & Number of observations & Mean Claim Amount & Sd of Claim Amount & Mean exposure \\ \hline
         0 & $397779$ & 0 & 0 & $0.555$ \\
         1 & $14633$ & $2041$ & $18734$ & $ 0.707$ \\
         2 & $726$ & $3033$ & $26506$ & $0.716$ \\
         3 & $28$ & $2170$ & $3838$ & $ 0.667$\\
         4 & $3$ & $1240$ & $167$ & $0.31$
    \end{tabular}
    \caption{Summary statistics for the claim amount and the exposure based on the number of claims. {\color{orange} Add Median}}
    \label{tab:sumstat}
\end{table}
We only consider the data where the number of claims is larger than zero. The data-set then contains $15390$ observations. We let $N_i$ denote the number of claims to policy i, and we let $Y_i$ denote the mean of the claims to policy i. Let $Y_{ij}$ denote the $j$'th claim to the $i$'th policy, and let $N_i$ be the total number of claims to one policy. We then have
\begin{equation*}
    Y_i = \dfrac{1}{N_i}\sum_{i=1}^{N_i} Y_{ij}.
\end{equation*}
Figure \ref{fig:HistData} shows histograms of $\mathbf{Y} = \{Y_i\}$ and $\mathbf{N} = \{N_i\}$
\begin{figure}[H]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/YHistogram.eps}
\caption{Histogram of $\mathbf{Y} = \{Y_i\}$}\label{fig:YHist}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/NHistogram.eps}
\caption{Histogram of $\mathbf{N} = \{N_i\}$} \label{fig:NHist}
\end{subfigure}
\caption{Histograms of $\mathbf{Y}= \{Y_i\}$ and $\mathbf{N} = \{N_i\}$}
\label{fig:HistData}
\end{figure}
We seek to model the joint distribution of $(\mathbf{N},\mathbf{Y})$, we investigate the dependence between these two variables. The correlation is fairly low
\begin{equation*}
    \text{cor}(\mathbf{Y},\mathbf{N}) = 0.011.
\end{equation*}
Figure \ref{fig:BoxplotClaims} shows a boxplot of the mean claim-amount for each policy as a function of the number of claims.
\begin{figure}[H]
    \centering
    \includegraphics[width = 0.6\linewidth]{fig/BoxplotClaims.eps}
    \caption{Boxplot of the mean claim amount for each policy as a function of the number of claims. The plot was cropped to get a better view, and as a result $613$ values where removed from the plot.}
    \label{fig:BoxplotClaims}
\end{figure}
Table \ref{tab:sumstat} and figure \ref{fig:NHist} reveals that the distribution of the number of claims, $\mathbf{N}$, is very skewed with the vast majority ($0.95)$ of the observations having $N_i = 1$. More problematically the distribution of the mean claim amounts seems to be heavy-tailed based on figure \ref{fig:YHist} and \ref{fig:BoxplotClaims}. It therefore seems reasonable to consider a logarithmic transformation of the claims instead
\begin{equation*}
    (lY)_i = \dfrac{1}{N_i} \sum_{i}^{N_i} \log(Y_{ij}+1).
\end{equation*}
We might also take the exposure into account and consider
\begin{equation*}
    (lEY)_i = \dfrac{1}{N_i} \sum_{i}^{N_i} \log\left(\dfrac{Y_{ij}}{E_i}+1\right),
\end{equation*}
where $E_i$ is the exposure of the $i$'th policy. Figure \ref{fig:HistTransData} shows histograms of respectively .. 
\begin{figure}[H]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/lYHistogram.eps}
\caption{Histogram of $\mathbf{lY}$}\label{fig:lYHist}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/lEYHistogram.eps}
\caption{Histogram of $\mathbf{lEY}$} \label{fig:lEYHist}
\end{subfigure}
\caption{Histograms of the two transformations of the data-set.}
\label{fig:HistTransData}
\end{figure}
Figure \ref{fig:BoxTransData} shows boxplots of $\mathbf{lY}$ and  $\mathbf{lEY}$. 
\begin{figure}[H]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/BoxplotlY.eps}
\caption{Boxplot of $\mathbf{lY}$}\label{fig:lYBox}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/boxplotlEY.eps}
\caption{Boxplot of $\mathbf{lEY}$} \label{fig:lEYBox}
\end{subfigure}
\caption{Histograms of the two transformations, $\mathbf{lY}$ and $\mathbf{lEY}$ of the data-set. Even though the data is log-transformed, there seems to be a problem with heavy-tails.}
\label{fig:BoxTransData}
\end{figure}
\begin{table}[H]
    \centering
    \begin{tabular}{c|c c}
         Phases & loglik & Iterations  \\ \hline
         10 & -29942.54 & 1000\\
         20 & 27399.32 & 4000 \\
    \end{tabular}
    \caption{Fitting just y}
    \label{tab:my_label}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabular}{c|c c}
        Phases & Loglik & Iterations  \\ \hline
        10 & -1930.699 & 1000 \\
        20 & -1760.411 & 4000
    \end{tabular}
    \caption{Small example fitting just y. Using different set of iterations to ensure convergence.}
    \label{tab:my_label}
\end{table}

{\color{orange}[MB: The distribution (based on the boxplot) seems to be heavy tailed. One can confirm this with a Hill plot. Probably considering $Y$ as mean of the logarithm of the claim amount might be better. The results regarding the log-likelihood are somewhat puzzling: they go up and down when increasing dimension. Also, we arrive at a worse log-likelohood than the independence model? We might want to incorporate exposure as well. So consider $Y_1=\sum_{i=1}^N\log(1+Y_i/exposure)/N$ and $N_1=N$, and model $(Y_1,N_1)$ instead of $(Y,N)$]}

\subsection{Interpretation}

\subsection{Fitting the Model}
\begin{itemize}
    \item Investigate how large a model is needed to capture data (on smaller data-set perhaps). 
    Especially Y seems to need a lot of phases
    \item Investigate if dependent model works better than independent (question of number of phases). Should we count total number of phases or dimension of marginal distributions?
    \item Plot log-likelihood as a function of parameters
    \item Investigate if other data-set has less problems with exposure. 
    \item Simulation study to check if independent model may be better with same amount of phases (getting more parameters) when splitting up. 
\end{itemize}

\begin{table}[H]
    \centering
    \begin{tabular}{c c|c c c | c c c }
        Phases & $\abs{E^+}$ &  \multicolumn{3}{c|}{Joint Model} &   \multicolumn{3}{c}{Independent Model}\\
        & & Joint log-lik & log-lik: $\mathbf{y}$ & log-lik: $\mathbf{n}$ & Joint log-lik (sum)& log-lik: $\mathbf{y}$ & log-lik: $\mathbf{n}$ \\ \hline
        5 & 2 & $-128967.3$ & $-125853.1$ & $ -3151.008$ & $-128328.5$ & $-125113.7$ & $ -3214.788$
    \end{tabular}
    \caption{Caption}
    \label{tab:FullData}
\end{table}




and in that way it is not the most obvious data-set to model using a bivariate model. {\color{red}[MB: Great work, Clara. I actually think this is a good dataset to model. The strength of our model is the interpretation one can give to the final fitted model, in terms of traversing states (causal representation). Correlation makes little sense when one variable takes only $0-4$ values. Perhaps a box-plot is better. However, if the final fitted model shows that the dependence structure of $(Y,N)$ is close to independence, this is also a good insight. There is also the second dataset of freMTPLsev2, and also the freMPL datasets (without the T). I would guess one of them should have some dependence - though I have no intuition yet since this approach has not been take before.]} \\
 
First we investigate how large a model is needed to model the data. As the data-set is fairly large we sample $1000$ observations from the data-sets. For this smaller data-set we use the EM-algorithm described in section... to fit models of different sizes to the data. 

\begin{table}[H]
    \centering
    \begin{tabular}{c c|c c c}
        Number of phases & $\abs{E}^+$ & Joint log-likelihood & Marginal log-likelihood: $\mathbf{y}$ & Marginal log-likelihood: $\mathbf{n}$  \\ \hline
        5 & 2 & $-8311.524$ & $ -8089.593$ & $ -227.5966$\\
        6 & 2 & $-8277.741$ & $-8056.247$ & $-227.4227$\\
        7 & 2 & $-8261.868$ & $-8040.461$ & $-227.4303$\\ 
        8 & 2 & $-8484.404$ \\
        9 & 2 & $-8448.524$ \\
        10 & 2 & $-8457.533$ \\
        11 & 2 & $-8424.962$ & $-8103.912$ & $-503.178$ \\
        20 & 2 & $-8393.069$ & $ -8073.895$ & $ -1679.911$\\
    \end{tabular}
    \caption{The log-likelihood after $1000$ for iterations for models with a different number of phases.}
    \label{tab:my_label}
\end{table}

{\color{red}[MB: 
When writing up the story we should just be careful to highlight that the time spent until each claim arrival is a latent proxy to the claim sizes, but not the claim sizes themselves. For a model where we include individual claim sizes into the estimation procedure, a Jamaal-approach would be better suited. Maybe we could have a chat with him at some point, out of curiosity. However, that is a different direction which we should not pursue in this paper. 
]}
\begin{figure}[H]
    \centering
    \includegraphics[width = 0.8 \linewidth]{fig/FittingY.eps}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


==> Thrash.tex <==


To proceed we now condition on the next state, $\tilde{Z}_{i+1}$. 
\begin{align*}
    \mathbb{E}\left[Y \mid N = n\right] & = \dfrac{1}{\text{P}\left[N = n\right]} \sum_{i=1}^n \sum_{j \in E^+} \sum_{k \in E^{+}}\text{P}\left[N=n \mid \tilde{Z}_{i+1} = k, \tilde{Z}_i = j\right] \text{P}\left[\tilde{Z}_i = j\mid \tilde{Z}_{i+1} = k\right] \cdot \mathbb{E}\left[ V_{ji} \mid, \tilde{Z}_{i+1} = k, N = n \right] \\
    &\cdot \text{P}\left[\tilde{Z}_{i+1} = k \mid N = n\right]
\end{align*}


To proceed we now condition on the next state visited in $E^+ \cup \{p+1\}$
\begin{align}
\begin{split}
    \mathbb{E}\left[ Y \mid N = n\right] &= \sum_{i=1}^n \sum_{j \in E^+} \mathbb{E}\left[\mathbf{1}_{\tilde{Z}_i = j} \cdot  V_{ji} \mid N = n \right] \\
    & =  \sum_{i=1}^{n-1} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{E}\left[\mathbf{1}_{\tilde{Z}_i = j} \cdot  V_{ji} \mid N = n , \tilde{Z}_{i+1} = k\right] \cdot \text{P}\left[\tilde{Z}_{i+1} = k \mid N = n\right] \\
    &= \sum_{i=1}^{n} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \text{P}\left[\tilde{Z}_i = j  \mid N = n , \tilde{Z}_{i+1} = k\right] \cdot \mathbb{E}\left[ V_{ji} \mid N = n , \tilde{Z}_{i+1} = k\right] \cdot \text{P}\left[\tilde{Z}_{i+1} = k\mid N = n\right] \\
    &= \sum_{i=1}^{n} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \dfrac{\text{P}\left[\tilde{Z}_i = j , N = n, \tilde{Z}_{i+1}=k \right]}{\text{P}\left[N = n, \tilde{Z}_{i+1}=k\right]} \cdot \mathbb{E}\left[ V_{ji} \mid N = n , \tilde{Z}_{i+1} = k\right] \cdot \text{P}\left[\tilde{Z}_{i+1} = k\mid N = n\right] \\
    \end{split} \label{eq:CondExpY}
\end{align}

To calculate $\text{P}\left[\tilde{Z}_i = j \mid N = n, \tilde{Z}_{i+1}=k\right]$ we write
\begin{align*}
    \text{P}\left[\tilde{Z}_i = j \mid N = n, \tilde{Z}_{i+1}=j\right]
    &= \dfrac{\text{P}\left[\tilde{Z}_i = j , N = n, \tilde{Z}_{i+1}=k \right]}{\text{P}\left[N = n, \tilde{Z}_{i+1}=k\right]} \\
    &=\begin{cases} \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right) \cdot  \tilde{Q}_{jk} \cdot\left( \mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{i} \mathbf{e}_k\right) \cdot \left(\mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)} \quad & \text{if } i< n-1 \text{ and } k \in E^+ \\
    \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1}\mathbf{e}_k\right) \tilde{Q}_{jk} \tilde{q}_{k}}{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{i} \mathbf{e}_k\right) \cdot \tilde{q}_k} \quad & \text{if } i = n-1 \text{ and } k \in E^+\\
    \dfrac{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}^{i-1}} \mathbf{e}_k \tilde{q}_k}{\tilde{\boldsymbol{\alpha}}\mathbf{Q}^{i-1} \mathbf{q}} \quad & \text{if } i = n \text{ and } k = p+1 \\
    0 \quad & \text{else}.
    \end{cases}
\end{align*}
To calculate $\mathbb{E}\left[V_{ji} \mid N = n\right]$, we first note that $V_{ji}$ follows a phase-type distribution with representation
\begin{align*}
    \boldsymbol{\beta} &= \begin{pmatrix} 1 & 0 & 0 & \cdots & 0 \end{pmatrix} \\
    \mathbf{T}_j&= \begin{pmatrix} s_{jj} & \mathbf{S}^{+0}_{j} \\
    \mathbf{0} & \mathbf{S}^{00}\end{pmatrix},
\end{align*}
where $\mathbf{S}^{+0}_{j}$ is the row of  $\mathbf{S}^{+0}$ corresponding to state $j$. To calculate $\mathbb{E}\left[V_{ij} \mid N = n, \tilde{Z}_{i+1} = k\right]$, we first note that given the next state $V_{ij}$ is independent of $N$
\begin{align*}
    \mathbb{E}\left[V_{ij} \mid \tilde{Z}_{i+1} = k\right].
\end{align*}
What we are looking at here, is the conditional expectation of a phase-type distribution conditioning on the absorption state. In \cite{CondPH} expressions for this is given. Let $\mathbf{t}_k$ be the absorption rate into state $k$. We then have
\begin{align*}
    \mathbb{E}\left[V_{ij} \mid \tilde{Z}_{i+1} = k\right] =  \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k}.
\end{align*}
At last we have
\begin{align*}
    \text{P}\left[\tilde{Z}_{i+1} = k \mid N = n\right] &= \dfrac{\text{P}\left[\tilde{Z}_{i+1} = k, N = n \right]}{\text{P}\left[N = n \right]} \\
    &= \begin{cases}\dfrac{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{i} \mathbf{e}_k\right) \cdot \left(\mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \quad & \text{if } i< n-1 \text{ and } k \in E^+ \\
    \dfrac{\left(\tilde{\boldsymbol{\alpha}} \mathbf{Q}^{i} \mathbf{e}_k\right) q_k}{\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{n-1}\tilde{\mathbf{q}}} \quad & \text{if } i = n-1 \text{ and } k \in E^{+} \\
    1 & \quad \text{if } i = n \text{ and } k = p+1 \\
    0 & \quad \text{else}
    \end{cases}
\end{align*}
Plugging into the expression in \eqref{eq:CondExpY} we obtain
\begin{align*}
    \mathbb{E}\left[Y \mid N = n\right] &= \sum_{i=1}^{n-2} \sum_{j \in E^+} \sum_{k \in E^+} \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right) \cdot  \tilde{Q}_{jk} \cdot\left( \mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{i} \mathbf{e}_k\right) \cdot \left(\mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k} \dfrac{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{i} \mathbf{e}_k\right) \cdot \left(\mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\tilde{\boldsymbol{\alpha}}  \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \\
    &+ \sum_{j \in E^+} \sum_{k \in E^+}     \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-2}\mathbf{e}_k\right) \tilde{Q}_{jk} \tilde{q}_{k}}{\left(\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{n-1} \mathbf{e}_k\right) \cdot \tilde{q}_k} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k} \cdot \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \mathbf{e}_k\right) \tilde{q}_k}{\tilde{\boldsymbol{\alpha}}\tilde{\mathbf{Q}}^{n-1}\tilde{\mathbf{q}}} \\
    &+ \sum_{j \in E^+}    \dfrac{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}^{n-1}} \mathbf{e}_k \tilde{q}_k}{\tilde{\boldsymbol{\alpha}}\mathbf{Q}^{n-1} \mathbf{q}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_{p+1}}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_{p+1}} \\
    &=\sum_{i=1}^{n-2} \sum_{j \in E^+} \sum_{k \in E^+} \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right) \cdot  \tilde{Q}_{jk} \cdot\left( \mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\tilde{\boldsymbol{\alpha}}  \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k} \\
    &+ \sum_{j \in E^+} \sum_{k \in E^+}     \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-2}\mathbf{e}_k\right) \tilde{Q}_{jk} \tilde{q}_{k}}{\tilde{\boldsymbol{\alpha}}  \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k}  \\
    &+ \sum_{j \in E^+}    \dfrac{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}^{n-1}} \mathbf{e}_k \tilde{q}_k}{\tilde{\boldsymbol{\alpha}}\mathbf{Q}^{n-1} \mathbf{q}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_{p+1}}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_{p+1}} \\
     &=\sum_{i=1}^{n-1} \sum_{j \in E^+} \sum_{k \in E^+} \dfrac{\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right) \cdot  \tilde{Q}_{jk} \cdot\left( \mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)}{\tilde{\boldsymbol{\alpha}}  \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k} \\
    &+ \sum_{j \in E^+}    \dfrac{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}^{n-1}} \mathbf{e}_k \tilde{q}_k}{\tilde{\boldsymbol{\alpha}}\mathbf{Q}^{n-1} \mathbf{q}} \cdot \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_{p+1}}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_{p+1}}.
\end{align*}    
The first term in this conditional expectation rather resembles the conditional expe



We now define the matrix $\mathbf{B}^{(i)}$ as
\begin{equation*}
    \mathbf{B}^{(i)} = \left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1}\right)' \left(\tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}} \right)',
\end{equation*}
for $i \in \{1,2,\ldots, n-1\}$. We have that $\mathbf{B}^{(i)}_{jk} =\left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right) \left( \mathbf{e}_k \tilde{\mathbf{Q}}^{n-i-1} \tilde{\mathbf{q}}\right)$, meaning that we can write the first term in the conditional expectation as
\begin{align*}
\dfrac{1}{\tilde{\boldsymbol{\alpha}}  \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \sum_{i=1}^{n-1} \sum_{j \in E^{+}} \sum_{k \in E^{+}} \mathbf{B}^{(i)}_{jk} \tilde{Q}_{jk} \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k}.
\end{align*}
TH\\




First we try to describe $(\mathbf{Y},\mathbf{N})$ by fitting the joint model to the data. The minimum value of $\mathbf{Y}$ was 250. Phase-type distributions are in general most suited for data-sets, which "starts" immediately at 0, and therefore we subtract the minimum and add 1
\begin{align*}
    \tilde{Y}_i = Y_i - \min(\mathbf{Y}) + 1.
\end{align*}
We experimented with the number of total phases in the phase-type distribution, $p$, and the number of phases counting in the discrete distribution, $\abs{E^+}$.For each combination of $(p, \abs{E^+})$ we fitted the joint model using the EM-algorithm described in section \ref{sec:Estimation}. The number of steps in the EM-algorithm was $10000$. For each fitted distribution we calculated the marginal distributions of the fit, such that we could also find the marginal likelihoods. To investigate whether the joint model was suitable we also fitted an independent model of approximately the same size as the joint model. A joint model with $p=i$ and $\abs{E^+} =j$ was compared to a phase-type distribution with $p=i$ phases and a discrete phase-type distribution with $p = j$ phases. This means that the independent model had more free parameters than the joint model. Assuming that the joint model starts in one of the states counting towards the discrete distribution (to avoid observations with $N_i=0$ and $Y_i >0$) the joint model has $j +i^2$ parameters, while the independent model has $j + j^2 + i + i^2$ parameters. \\

Table \ref{tab:SweYResults} summarizes the results of fitting joint and independent phase-type models to the data-set. 
\begin{table}[H]
    \centering
    \begin{tabular}{c c|c c c | c c c}
        \multirow{2}{*}{p} & \multirow{2}{*}{$\abs{E^+}$} & \multicolumn{3}{c |}{Joint Model} & \multicolumn{3}{c}{Independent Model} \\ 
        & & Joint loglik & Y loglik & N loglik & Sum loglik & Y loglik & N loglik \\ \hline
        \multirow{1}{*}{2}& $1$ & $-7394.453$ & $-7276.752$ & $-114.0873$ & $-7389.907$ & $-7275.820$ & $-114.0873$ \\ \hline
        \multirow{2}{*}{3} & $1$ & $-7383.499$ & $-7275.369$ & $-114.0873$ &  $-7389.606$ & $-7275.518$ & $-114.0873$ \\
        & 2 & $-7382.494$ & $-7275.546$ & $-113.5011$ & $-7388.511$ & $-7275.518$ & $-112.9924$ \\   \hline
        \multirow{3}{*}{4} & $1$ & $-7382.352$ & $-7275.066$ & $-114.0873$ & $-7386.421$ & $-7272.333$ & $-114.0873$ \\ 
        & $2$ & $-7381.660$ & $-7275.513$ & $-112.9924$ & $-7385.326$ & $-7272.333$ & $-112.9924$ \\
         & 3 & $-7379.213$ & $-7273.052$ &  $-113.1312$ & $-7385.326$ & $-7272.333$ & $-112.9924$ \\ \hline
        \multirow{3}{*}{5} & $1$ & $-7378.938$ & $-7271.755$ & $-114.0873$ & $-7386.409$ & $-7272.322$ & $-114.0873$ \\
        & $2$ & $-7377.750$ & $-7271.699$ & $-113.0340$ & $-7385.315$ &  $-7272.322$ & $-112.9924$ \\
        & $3$ & $-7378.098$ &  $-7272.111$ & $-113.1233$ & $-7385.315$ & $-7272.322$ & $-112.9924$ \\ \hline
        \multirow{3}{*}{6}& $1$ & $-7377.063$ & $-7268.901$ & $-114.0873$ & $-7389.602$ & $-7275.515$ & $-114.0873$ \\
        & $2$ &  $-7376.840$ & $-7270.938$ & $-113.1183$ & $-7388.507$ & $-7275.515$ & $-112.9924$ \\
        & $3$ & $-7377.647$ & $-7271.678$ & $-113.1237$ & $-7388.507$ & $-7275.515$  & $-112.9924$ \\ \hline
        \multirow{3}{*}{7} & $1$ & $-7375.617$ & $-7267.833$ & $-114.0873$ & $-7383.409$ & $-7269.322$ & $-114.0873$ \\
        & $2$ & $-7376.746$ & $-7270.653$ & $-112.9924$ & $-7382.314$ & $-7269.322$ & $-112.9924$ \\
        & $3$ & $-7376.394$ & $-7270.759$& $-112.9996$ & $-7382.314$ & $-7269.322$ & $-112.9924$ \\ \hline
        \multirow{3}{*}{8} & $1$ & $-7375.597$ & $-7267.634$ & $-114.0873$ & $-7383.174$ & $-7269.087$ & $-114.0873 $ \\
        & $2$ & $-7374.930$ & $-7269.339$ & $-112.9924$ & $-7382.079$ & $-7269.087$ & $-112.9924$ \\
        & $3$& $-7376.095$ & $-7270.032$ & $-112.9924$ & $-7382.079$ & $-7269.087$ & $-112.9924$ \\ \hline
        \multirow{3}{*}{9} & $1$ & $-7377.579$ & $-7269.988$ & $-114.0873$ & $-7384.113$ & $-7270.026$ & $-114.0873$ \\        & $2$ & $-7378.142$ & $-7272.466$ & $-112.9924$ & $-7383.018$ & $-7270.026$ & $-112.9924$ \\
        & $3$ & $-7380.346$ & $-7274.408$ & $-112.9924$ & $-7383.018$ & $-7270.026$ & $-112.9924$ \\ \hline 
        \multirow{3}{*}{10} & $1$ & $-7373.488$ & $-7266.324$ &  $-114.0873$ & $-7382.726$ & $-7268.639$ & $-114.0873$ \\
        & $2$ & $-7381.395$ & $-7275.279$ & $-112.9924$ & $-7381.631$ & $-7268.639$ & $-112.9924$ \\
        & $3$ & $-7381.431$ & $-7275.332$ & $-112.9924$ & $-7381.631$ & $-7268.639$ & $-112.9924$
    \end{tabular}
    \caption{Likelihoods of fits for a joint phase-type distribution and two independent phase-type distributions. The fits were obtained using the EM-algorithm with $10000$ iterations. For all parameter combinations, except the first one, the likelihood of the joint model is higher than the likelihood of the independent model}
    \label{tab:SweYResults}
\end{table}
Figure \ref{fig:SweYRes} shows a plot of the results in \ref{tab:SweYResults}, which makes it easier to interpret the results
\begin{figure}[H]
    \centering
    \includegraphics[width = 0.8 \linewidth]{fig/SweMb/SweYLikelihoodplot.eps}
    \caption{The log-likelihood of the fit for different model sizes. The dotted lines shows the joint model and the solid lines shows the independent model. For the joint model we see the expected increase in the likelihood with the number of total phases until $p = 8$. Hereafter a small decrease is seen, which is probably because too few steps were used in the EM-algorithm. There is no clear trend regarding the number of phases in $E^+$, suggesting that this number has less importance. For the independent model the likelihood also increases with the number of phases - both in the continuous and the discrete distribution. It is seen that is does not matter if $2$ or $3$ phases are used, which is because the maximum amount of claims is $2$.}
    \label{fig:SweYRes}
\end{figure}
Based on these figures, it is evident that the joint model is more suited to describe $(\mathbf{Y},\mathbf{N})$. We can make the picture even more clear by taking the number of parameters into account. Figure \ref{fig:SweYPars} shows two ways of doing this. 

\begin{figure}[H]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/SweMb/sweYParLoglik.eps}
\caption{The log-likelihood of the different fitted models as a function of the number of parameters. The independent models have more parameters than the correspoding joint models}\label{fig:SweYParll}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/SweMb/sweYAIC.eps}
\caption{The AIC of the different fitted models. From this plot the preffered model seems to be the joint model with $p = 3$ and $\abs{E^+} = 2$. The AIC is generally lower for the joint model} \label{fig:SweYAIC}
\end{subfigure}
\caption{The log-likelihood as a function of the number of parameters, and the AIC of the different fits. }
\label{fig:SweYPars}
\end{figure}

\subsection{Post-Hoc Analysis}
Based on figure the results in .. we can choose the best model to describe the data. Based on the AIC the best model is.. However for the sake of illustration we also continue with a slightly larger model which has better likelihood and more parameters, which highlights some of the advantages of our joint model.

\subsubsection{Conditional Distributions}
The joint model of $(\mathbf{Y}, \mathbf{N})$ allows us to find a  phase-type representation of the conditional distribution of $Y \mid N$ as described in section \ref{sec:ConditionalDist}. This sheds some light on the influence of the number of claims. 

For the model with $p = 5$ and $\abs{E^+} = 2$, we calculate the conditional densities and distribution function. 

Figure \ref{fig:CondDens} shows the result along with a histogram of the data, and figure \ref{fig:CondDist} shows the distribution function along with the empirical distribution function

\begin{figure}[H]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/SweMb/CondPlotSweY.pdf}
\caption{The conditional distribution of $Y$ given $N$ along with histograms of the corresponding data.\\ \\ \\ \\}\label{fig:CondDens}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{fig/SweMb/CondDistSweY.pdf}
\caption{The conditional distribution functions obtained from the fit, and the empirical distribution function for $1$ and $2$ claims respectively. For $1$ claim the maximum distance between the two distribution functions is $D_1 = 0.032$ and for $2$ claims the maximum distance between the two distribution functions is $D_2 = 0.054$.} \label{fig:CondDist}
\end{subfigure}
\caption{}
\label{fig:CondDist}
\end{figure}
We can also calculate the conditional expectations. 

\subsubsection{Pure Premium}
The main advantage of the joint model, is that it allows us to calculate the pure premium $\mathbf{E}\left[Y N\right]$ without an assumption of independence between $Y$ and $N$. Using the model with $p=5$ and $\abs{E}^+ = 2$, we can calculate the pure premium as
\begin{equation*}
    \mathbb{E}\left[Y N \right] = -25415.65.
\end{equation*}
If we instead fit two independent models - one continuous phase-type distribution with $p = 5$ and one discrete phase-type distribution with $p = 2$, we obtain the following pure premium
\begin{equation*}
    \mathbb{E}\left[Y N\right] = \mathbb{E}\left[Y\right] \cdot \mathbb{E}\left[N\right] = 23769.21 \cdot  1.04 = 24732.83
\end{equation*}
The true pure-premium for the data is $25421.4$. A standard confidence interval can be calculated to be $[25307.45, 25535.35]$, which includes the result from the joint model, but not the result from the independent model.

\subsection{Australian Car Insurances}
The \texttt{swmotorcycle} data-set is a premium data-set to highlight the advantages of our model. Due to the high correlation between $N$ and $Y$ the dependent model described the data better than the independent models. Also the pure premium was estimated more correctly using the dependent model. In this section we will consider a data-set, where the independence assumption is not as far-fetched, and investigate how our model fares. \\


\subsection{Data Description}
We will consider the data-set \texttt{ausprivauto0405} from the R-package \texttt{CASdatasets}. The data-set consists of $4624$ policies. Table \ref{tab:sumaus} contains summary statistics
\begin{table}[H]
    \centering
    \begin{tabular}{c|c c c c c c c}
        \# Claims & Mean of $\mathbf{y}$ & Median of $\mathbf{y}$ & Sd of $\mathbf{y}$ &  Mean of $\mathbf{ye}$ & Median of $\mathbf{ye}$ & Sd of $\mathbf{ye}$ & \# of obs \\ \hline
        1 &  1748 &  497 &  3547 &  11299 & 1123 & 123056 &  4333 \\
        2  & 1273 & 654 &  1732 &   2186 & 1074 & 3304 &  271 \\
        3  & 1142 & 770 & 943 & 2092 & 1335 & 2506 & 18 \\
        4 & 911 & 911 & 736 & 1077 & 1077 & 894 & 2
    \end{tabular}
    \caption{Summary statistics of \texttt{ausprivauto0405} based on the number of claims}
    \label{tab:sumaus}
\end{table}

Investigate which states we visit in the conditional distributions.

Maybe not include australian data, but look at exposure and not exposure? Gives to very different results because of the lack of dependency

\section{Discussion}
Estimation procedure. The EM-algorithm depends a lot on the number of iterations. Some of the fits might not be completely converged. Since differences in likelihood are so small, we might have problem comparing.

Problems modelling exposure with australian data.

\subsection{Estimation Issues}
Calculate likelihood in R instead? For Y also. Investigate how much likelihood we gaing for more steps in the simulation procedure (plot to see when we can stop). See if it changes, if we supply the estimated Y rep as start-guess (and see if it changes the likelihood).

Ideas for further investigations:
\begin{itemize}
    \item Switch n = 1 and n = 2, and see what happens if we have dependence the other way around.
    \item Try to create more balanced data-set. Sample more obs with $n = 2$. How to do that?
\end{itemize}
\subsection{Conditional Expectations} \label{sec:CondExp}
{\textcolor{red}{I think we should delete this section and possibly make it into a small note in the section above.}}

We now seek to calculate the conditional expectation $\mathbb{E}\left[Y \mid N = n\right]$. We write out $Y$ as a stochastic sum based on the embedded Markov chain
\begin{equation*}
    Y = \sum_{i=1}^{\infty} \sum_{j=1}^p\mathbf{1}_{Z_i = j} W_{ji},
\end{equation*}
where $p = \abs{E}$ and $W_{ji} \sim \exp(-s_{jj})$. When conditioning on $N$ it is beneficial to split the sum of the states into the states belonging to $E^+$ and $E^0$. We then have
\begin{equation*}
    Y = \sum_{i=1}^{\infty} \sum_{j \in E^+}\mathbf{1}_{Z_i = j} W_{ji} + \sum_{j \in E^0}\mathbf{1}_{Z_i = j} W_{ji}.
\end{equation*}
As we condition on $N=n$ we have that the number of visits to the states in $E^+$ has to equal $n$. The Discrete Markov Chain $\{\tilde{Z}_{n}\}_{n \in \mathbb{N}}$ counts the number of visits to these states. If we let $Y^{(+)}$ denote the contribution from states in $E^+$ to $Y$ and $Y^{(0)}$ denote the contribution to $Y$ from state in $E^0$, then we have
\begin{align*}
    Y^{(+)} = \sum_{i=1}^{\infty} \sum_{j \in E^+}\mathbf{1}_{\tilde{Z}_i = j} W_{ji}
\end{align*}
As we want to condition on $N$ it is beneficial to keep counting the states using $\{\tilde{Z}_n\}_{n \in \mathbb{N}}$. We note now that every visit to a state in $E^+$ may be followed by a visit to one or more states in $E^0$. Let $Y^{(0)}_{i,j}$ be the contribution from states in $E^0$ following $\tilde{Z}_i$ given $\tilde{Z}_i = j$. We then define
\begin{equation*}
    V_{ji} = W_{ji} + Y^{(0)}_{i,j}.
\end{equation*}
Note that $Y^{(0)}_{i,j} = 0$ is possible if there is no visits to states in $E^0$. We can now write
\begin{equation*}
    Y = \sum_{i=1} \sum_{j \in E^+} \mathbf{1}_{\tilde{Z}_i = j} V_{ji}.
\end{equation*}
We also consider a slightly different version of $V_{ji}$. First note that $V_{ji}$ is a phase-type distribution on the states $j \cup E^0$. This phase-type distribution can absorb into all the states in $E^+$ and into state $p+1$. We now consider $V_{jki}$, which is given as
\begin{equation*}
    V_{jki} = W_{ji} + Y_{i,j,k}^{(0)},
\end{equation*}
where $Y_{i,j,k}^{(0)}$ is the contribution from states in $E^0$ following $\tilde{Z}_i$ given $\tilde{Z}_i = j$ and $\tilde{Z}_{i+1} = k$.
We can then write
\begin{equation*}
    Y = \sum_{i=1} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}}\mathbf{1}_{\tilde{Z}_i = j} \cdot \mathbf{1}_{\tilde{Z}_{i+1} = k} \cdot V_{jki}
\end{equation*}
Taking the conditional expectation of $Y$ then amounts to
\begin{align*}
    \mathbb{E}\left[ Y \mid N = n\right] &= \sum_{i=1}^n \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{E}\left[\mathbf{1}_{\tilde{Z}_i = j} \cdot \mathbf{1}_{\tilde{Z}_{i+1} = k}\cdot  V_{jki} \mid N = n \right] \\
    &=  \sum_{i=1}^n \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{P}\left[\tilde{Z}_i = j \cdot \tilde{Z}_{i+1} = k\mid N = n\right]\cdot \mathbb{E}\left[ V_{jki} \mid N = n \right] \\
   &=\sum_{i=1}^n \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{P}\left[\tilde{Z}_i = j \cdot \tilde{Z}_{i+1} = k\mid N = n\right]\cdot \mathbb{E}\left[ V_{jki} \right]
\end{align*}
where we have used that $\mathbf{1}_{\tilde{Z}_i = j} \cdot \mathbf{1}_{\tilde{Z}_{i+1} = k}$ and $V_{jki}$ are independent as sojourn times are independent from jumps. Furthermore we have used that $V_{jki}$ is independent of $N$. Thus,
{\small
\begin{align*}
    &\mathbb{E}\left[ Y \mid N = n\right]\\ 
    &= \sum_{i=1}^{n} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \dfrac{1}{\mathbb{P}\left[N = n\right]} \cdot \mathbb{P}\left[ \tilde{Z}_i = j, \tilde{Z}_{i+1} = k, N = n\right] \cdot \mathbb{E}\left[ V_{jki} \right] \\
    &= \dfrac{1}{\mathbb{P}\left[N = n\right]} \cdot \sum_{i=1}^{n} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{P}\left[N = n \mid \tilde{Z}_{i+1} = k , \tilde{Z}_{i} = j\right] \mathbb{P}\left[\tilde{Z}_{i+1} =k \mid \tilde{Z}_{i} = j \right] \cdot \mathbb{P}\left[\tilde{Z}_i= j\right] \cdot \mathbb{E}\left[ V_{jki} \right] \\
    &= \dfrac{1}{\mathbb{P}\left[N = n\right]} \cdot \sum_{i=1}^{n} \sum_{j \in E^+} \sum_{k \in E^+ \cup \{p+1\}} \mathbb{P}\left[N = n \mid \tilde{Z}_{i+1} = k \right] \mathbb{P}\left[\tilde{Z}_{i+1} =k \mid \tilde{Z}_{i} = j \right] \cdot \mathbb{P}\left[\tilde{Z}_i= j\right] \cdot \mathbb{E}\left[ V_{jki} \right] \\
    &=\dfrac{1}{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \cdot \left(\sum_{i=1}^{n-1} \sum_{j \in E^+ } \sum_{k \in E^+} \left(\mathbf{e}_k' \tilde{\mathbf{Q}}^{n-1-i} \tilde{\mathbf{q}} \right) \tilde{Q}_{jk} \left(\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1} \mathbf{e}_j\right)\cdot \mathbb{E}\left[ V_{jki} \right] +\sum_{j \in E^+} \tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{q}_j \mathbb{E}\left[V_{j,p+1,n}\right] \right)
\end{align*}
}
%The first sum is a quantity that also arises in the EM algorithm for DPH-distributions. 
We let
\begin{equation*}
    \mathbf{K}(n) = \sum_{i=1}^{n-1} \tilde{\mathbf{Q}}^{n-1-i} \tilde{\mathbf{q}} \tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{i-1},
\end{equation*}
so that we may write
\begin{align*}
    \mathbb{E}\left[Y \mid N = n  \right]  = \dfrac{1}{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \left(K(n)_{kj} \tilde{Q}_{jk}  \mathbb{E}\left[ V_{jki} \right] +\sum_{j \in E^+} \tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{q}_j \mathbb{E}\left[V_{j,p+1,n}\right] \right).
\end{align*}
Using a discrete version of the classical Van Loan identity, we can calculate $\mathbf{K}$ matrix efficiently as
\begin{equation*}
    \begin{pmatrix} \tilde{\mathbf{Q}} & \tilde{\mathbf{q}} \tilde{\boldsymbol{\alpha}} \\ \mathbf{0} & \tilde{\mathbf{Q}} \end{pmatrix}^{n-1} = \begin{pmatrix}
    \tilde{\mathbf{Q}}^{n-1} & \mathbf{K}(n) \\ \mathbf{0} & \tilde{\mathbf{Q}}^{n-1}
    \end{pmatrix}.
\end{equation*}

Thus, it remains to calculate $\mathbb{E}\left[V_{jki}\right]$, the conditional expectation of a phase-type distribution conditioning on the absorption state, which may be found in \cite{CondPH}. Let $\mathbf{t}_k$ be the absorption rate into state $k$. We then have
\begin{align*}
    \mathbb{E}\left[V_{jki}\right] =  \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k}.
\end{align*}
Inserting this we obtain
\begin{equation*}
     \mathbb{E}\left[Y \mid N = n  \right]  =\dfrac{1}{\tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{\mathbf{q}}} \left(K(n)_{kj} \tilde{Q}_{jk} \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_k}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_k}+\sum_{j \in E^+} \tilde{\boldsymbol{\alpha}} \tilde{\mathbf{Q}}^{n-1} \tilde{q}_j \dfrac{\boldsymbol{\beta} \left( -\mathbf{T}_j\right)^{-2} \mathbf{t}_{p+1}}{\boldsymbol{\beta}\left(-\mathbf{T}_j\right)^{-1}\mathbf{t}_{p+1}}\right)
\end{equation*}


The other conditional expectation is easier to calculate, as the main calculation is done in the usual EM algorithm for phase-type distributions. We have
\begin{align*}
    \mathbf{E}\left[N_{ij}  \mid Y = y\right] &= \dfrac{t_{ij} \mathbf{e}_j' \int_{0}^y \exp\left(\mathbf{T}(y-u)\right) \mathbf{t}\boldsymbol{\alpha} \exp\left(\mathbf{T} y \right) du \mathbf{e}_i}{\boldsymbol{\alpha}\exp\left(\mathbf{T}y\right) \mathbf{t}}\\
    \mathbb{E}\left[N_i = \mid Y = y\right] &= \dfrac{\boldsymbol{\alpha}\exp\left( \mathbf{T}y\right) \mathbf{e}_i t_i}{\boldsymbol{\alpha}\exp\left( \mathbf{T}y\right) \mathbf{t}},
\end{align*}
where $N_{ij}$ is the number of jumps from state $i$ to state $j$, and $N_i$ is the number of jumps from state $i$ to the absorbing state, $p+1$.
We can now find $\mathbb{E}\left[N\mid Y = y\right]$ by counting the number of jumps from states in $E^+$ to other states
\begin{align*}
    \mathbb{E}\left[N \mid Y = y \right] = \sum_{i \in E^+} \sum_{j = 1}^{p} \mathbb{E}\left[N_{ij} \mid Y =y\right] + \mathbb{E}\left[N_i \mid Y = y\right].
\end{align*}
See Section \ref{sec:Estimation} for details on how to compute these quantities. 

